XSB: Extending Prolog with Tabled Logic Programming

The paradigm of Tabled Logic Programming (TLP) is now supported by a number of Prolog systems, including XSB, YAP Prolog, B-Prolog, Mercury, ALS, and Ciao. The reasons for this are partly theoretical: tabling ensures termination and optimal known complexity for queries to a large class of programs. However the overriding reasons are practical. TLP allows sophisticated programs to be written concisely and efficiently, especially when mechanisms such as tabled negation and call and answer subsumption are supported. As a result TLP has now been used in a variety of applications from program analysis to querying over the semantic web. This paper provides a survey of TLP and its applications as implemented in XSB Prolog, along with discussion of how XSB supports tabling with dynamically changing code, and in a multi-threaded environment.

==> knapsack.tex <==
\subsubsection{Knapsack example}

Next we consider the knapsack problem.  The idea is that we have a
knapsack and a bunch of things of various sizes to put in it.  The
question is whether there is a subset of the things that will fit
exactly into the knapsack.  The problem can be formally stated as
follows:

\begin{quote}
  Given $n$ items, each of integer size $s_i$ $(1 \le i \le n)$, and a
  knapsack of size S,  1) determine whether there is a subset of the
  items that sums to S, and optionally 2) if so, find such a subset.
\end{quote}

We number the items and represent them and their sizes by using a
set of facts \verb|item/2|, where, for example, \verb|item(3,5)| means
that the third item is of size 5.

To determine whether there is a subset of items that exactly fill the
knapsack, we can define a predicate, \verb|ks/2|, shown in Figure
\ref{fig:knapsack-rec}, that simply tries all alternatives 
nondeterministically. \verb|ks(ItemCnt,Size)| is true if there is a
subset of the items numbered 1 to \verb|ItemCnt| whose sizes sum to
\verb|Size|.

\begin{figure}[htbp]
\begin{center}
\begin{verbatim}
% ks(+K,+S) if there is a subset of items 1,...,K whoses sizes sum to S.
:- table ks/2.
ks(0,0).               % the empty set sums to 0
ks(K,S) :- K>0,        % choose not to include this Kth element in the knapsack
    K1 is K-1,
    ks(K1,S).          % if sizes of earlier items add to S
ks(K,S) :- K>0,        % choose to include this Kth element in the knapsack
    item(K,Sk),
    S1 is S-Sk, 
    S1 >= 0, 
    K1 is K-1, 
    ks(K1,S1).         % if sizes of earlier items add to S reduced by K's size
\end{verbatim}
\end{center}
\caption{TLP Program for the Knapsack Packing Problem}
\label{fig:knapsack-rec}
\end{figure}

The first clause says that the empty set takes no space in the sack.
The second clause covers the case in which the Kth item is {\em not}
included in the sack.  The third clause handles the case in which the
Kth item {\em is} included in the sack.

Under naive Prolog evaluation this program would be exponential in the
number of items, since it tries all subsets of items.  However, for
$n$ items and target size of $s$ there are only $n*s$ possible
distinct calls to \verb|ks/2|.  Thus adding the \verb|:- table ks/2|
declaration will make this polynomial in these parameters.

This predicate \verb|ks/2| finds only whether a packing of the
knapsack of a given size exists; it does not tell us what particular
set(s) of items we should include to have that exact fit.  The obvious
solution is to simply add a third argument to this definition of
\verb|ks/2| to maintain a list of the item numbers for items included
in the knapsack.  But the complexity of the resulting definition may
then be exponential.  Consider the case in which every item had a size
of $1$.  Then for each sum S (not greater than the number of items
$N$), there are $N choose~S$ ways to achieve it, creating that many
calls.  Of course, if we want all answers and there are exponentially
many, we will necessarily require exponential behavior.  But consider
the case in which we have $N$ items each of size 1, and we ask if
there is a knapsack of size $N+1$.  The answer is no, but our program
will take exponential time to come to that answer. 
\comment{
\dsw{WRONG!! They take
exponential time ONLY if there are exponentially many answers.  We
only make a call to ksp/3 if it is known that it can be extended to a
full answer. The thought now is to remove this example and replace it
with the grammar discussion below.}
}

To solve this problem, we can add the extra argument, but also use our
(polynomial) definition of \verb|ks/2| above to avoid unnecessary
computation.  Our definition of \verb|ksp/3| is shown in Figure
\ref{fig:knapsack-ways}.

\begin{figure}[htbp]
\begin{center}
\begin{verbatim}
% ksp(K,S,ItmLst) if the sizes of items (numbered <= K) in ItmLst sum to S
:- table ksp/3.
ksp(0,0,[]).
ksp(I,K,P) :- I>0,     % do *not* include Kth item
    I1 is I-1, 
    ks(I1,K),          % only if there is a packing
    ksp(I1,K,P).       % then go find it (or them)
ksp(I,K,[I|P]) :- I>0, % *do* include Kth item
    item(I,Ki), 
    K1 is K-Ki, 
    K1 >= 0, 
    I1 is I-1, 
    ks(I1,K1),         % only if there is a packing
    ksp(I1,K1,P).      % go find the ways
\end{verbatim}
\end{center}
\caption{TLP Program for Ways to Pack a Knapsack}
\label{fig:knapsack-ways}
\end{figure}

This program maintains the polynomial behavior, assuming only
polynomial ways to fill the knapsack.

This issue of a polynomial tabled predicate becoming exponential with
the addition of an extra argument arises in a variety of situations.
For example, in context-free language processing, adding an argument
to a recognizer to collect the parse tree may also introduce
extraneous exponentiality.  Recent work \cite{ChrG09} has developed
analysis and transformation techniques that can recognize when this
issue might arise for a tabled program, as in \verb|ksp/3|, and
automatically transform it to a possibly more efficient form.


==> parsing.tex <==

%\subsubsection{Example: Context-Free Parsing} \label{ex:parsing}
%\tls{Maybe a bit of motivation about the importance of parsing.  We're
%  already citing \cite{syntactica-semantica,CuSw02} and its also
%  relevant to the XSB Inc application}
%dsw{I've added a paragraph following this intro to address this.}

%\begin{example}[Context-Free Parsing] \label{ex:parsing}
{\em Example 2.3 (Context-Free Parsing\ )}
Prolog (and XSB) support Definite Clause Grammars (DCGs), a syntax for
representing context-free grammars using Prolog rules.  
%%One can use
%%DCG rules to recognize strings in the specified language.  
Prolog's
evaluation strategy applied to a DCG specification results in a
recursive descent recognition algorithm, with its attendant
disadvantages: it loops infinitely on left recursive grammars, and it
may have exponential complexity for grammars and strings it does
handle.  However, when tabled evaluation is applied to a DCG
specification (with no non-terminal parameters and in which every predicate representing a nonterminal is
tabled), the resulting algorithm is a chart parser (and a
variation of Earley's context-free language recognition
algorithm~\cite{Earl70}), which handles
all context-free grammars with polynomial complexity.
%%, with
%%even better complexity results for certain special classes of
%%grammars.

A number of applications use tabled grammars in XSB.  Two pedagogical
systems \cite{syntactica-semantica} use XSB grammars to teach natural
language syntax and semantics to linguistics students.  Several
applications in use by XSB, Inc., and described in
Section \ref{sec:applic}, depend crucially on tabled grammars.

Consider the following simple DCG, and the Prolog program it
generates:
{\small
\begin{verbatim}
s --> s, s.  % S -> SS                        % DCG
s --> a.     % S -> a

:- table s/2.
s(S0,S) :- s(S0,S1), s(S1,S).
s(S0,S) :- 'C'(S0,a,S).

% Prolog definition of connects predicate 'C'/2.
'C'([X|S],X,S).
\end{verbatim}
}
This is a left recursive context-free grammar, essentially the doubly
recursive version of transitive closure, and with the table
declaration XSB will correctly and polynomially handle recognition
queries such as:
{\small
\begin{verbatim}
?- s([a,a,a,a,a,a,a],[]).
\end{verbatim}
}
However, there is an unnecessary computational overhead due to the
list representation of the input.  Each tabled call to s/2 will copy
the list representing the remainder of the input string into the
table, which is inefficient as discussed for {\tt append/3} in
Section~\ref{sec:sched-eff}.  Here 
a list is used to represent a position in the input string,
which can be avoided by use of a different input representation.  When
tabled DCG's are used, XSB can represent an input string,
$s_1,s_2,...,s_n$, by a set of facts of the form $word(i-1,s_i,i)$ and
redefine the connects predicate to be:
{\small
\begin{verbatim}
'C'(S0,X,S) :- word(S0,X,S).
\end{verbatim}
}
With this datalog-style representation, integers represent positions
in the input string, and only integers, not lists, need to be copied to the
table.  %, thus removing the extra linear factor from the complexity.
Under the datalog-style representation, if we transform a grammar into
Chomsky form (where every rule has at most two terminal or nonterminal
symbols on its right-hand-side), tabled evaluation results in Earley's
recognition algorithm (i.e., for grammars with nonterminals with no arguments.)

%\dsw{I can't get suppl\_table to work in XSB, so I'm not adding a
%statement about it.}
\comment{XSB supports a directive \verb|:- suppl_table|, which
automatically transforms a grammar (or other program) into an
equivalent one in which has at most two predicate calls in the body of
any rule.  For grammars this guarantees cubic complexity as worst-case
for recognition.}

The above ``nonparameterized'' DCG specification performs language
recognition.  Often DCG users want to construct a parse tree (or
abstract syntax tree) for input strings and do this by adding to each
nonterminal predicate an extra argument in which the tree is
constructed.  For example, the specification:
{\small
\begin{verbatim}
:- table s/3.
s(s(P1,P2)) --> s(P1), s(P2).  % S -> SS      % DCG with parse tree
s(a) --> a.                    % S -> a
\end{verbatim}
}
shows how a term representing the parse tree for a recognized string
would be built for our simple grammar example.  This grammar has
exponentially many parse trees for each string it recognizes, so it
will take exponential time to find and produce them.  But if a string
is {\em not} in the language, we would hope to be able to determine that in
polynomial time (as the recognizer does.)  However, for
the string \verb|aaaaaaaaaab|, the above parser will produce all the
exponentially many sub-parses for the initial string of a's, only to
detect that none can be extended to a parse of the entire input
string.  
%So this will also take exponential time, even though no
%parses are produced.  
This can be fixed by using the previous tabled recognizer to condition
what parses are to be constructed.  For example,
{\small
\begin{verbatim}
s --> s, s.  % S -> SS           % DCG recognizer (non-tabled)
s --> a.     % S -> a

:- table s/3.                    % Prolog for parse tree, with filter
s(s(P1,P2),S0,S) :-  s(S0,S1),s(S1,S),s(P1,S0,S1),s(P2,S1,S).
s(a,S0,S) :- 'C'(S0,a,S).
\end{verbatim}
}
in the rules that construct the parse, we have called the recognition
rules to ensure that a parse exists for the entire string before
proceeding to construct the parse.  This set of rules now has the
complexity of the recognizer, plus linear time in the number of
parses.
%
The general problem of making a program linear in the number of
solutions it derives, even when there can be exponentially many, is
exhibited in other problems, such as in finding paths though graphs
and in combining the probabilities of subcomputations.  A recent
paper \cite{ChrG09} describes an algorithm to detect such situations,
and to automatically convert the exponential program into one with
better complexity.
%\end{example}


==> sld-full.tex <==
From a theoretical perspective SLD, the resolution method underlying
Prolog, is complete in that it generates a proof for every correct
answer for a query $Q$ to a program $P$.  At the same time, the search
for an SLD proof may not terminate, even when $P$ has the bounded
term-depth property (e.g., when $P$ is a datalog program).  For example,
consider the query {\tt ?- reach(1,Y)} to the program 
 $P_{Lrec}$ in Figure~\ref{fig:sldtree}.  An SLD search tree for this
query is also shown in Figure~\ref{fig:sldtree} where Prolog's
top-to-bottom clause selection strategy and left-to-right literal
selection strategy are both used.  Note that the tree contains proofs
of (i.e. root-to-leaf paths to) both of the correct answer
ubstitutions, $Y = 2$ and $Y = 3$, but that the tree is infinite and
both of these answers lay to the right of an infinite branch.
%
This accords with the behavior of Prolog
on this query and program: Prolog will go into an infinite loop before
deriving the first answer.  Indeed, since the tree is infinite, no
complete search will ever terminate.
%
\begin{figure}[htbp]
\centering
\epsfig{file=Figures/sldtree.eps,width=\textwidth}
\caption{A program $P_{Lrec}$ and SLD tree for the query {\em reach(1,Y)}}
\label{fig:sldtree}
\end{figure}


